Towards a Game-theoretic Understanding of Explanation-based Membership Inference Attacks

Model explanations improve the transparency of black-box machine learning (ML) models and their decisions; however, they can also be exploited to carry out privacy threats such as membership inference attacks (MIA). Existing works have only analyzed MIA in a single "what if" interaction scenario between an adversary and the target ML model; thus, it does not discern the factors impacting the capabilities of an adversary in launching MIA in repeated interaction settings. Additionally, these works rely on assumptions about the adversary's knowledge of the target model's structure and, thus, do not guarantee the optimality of the predefined threshold required to distinguish the members from non-members. In this paper, we delve into the domain of explanation-based threshold attacks, where the adversary endeavors to carry out MIA attacks by leveraging the variance of explanations through iterative interactions with the system comprising of the target ML model and its corresponding explanation method. We model such interactions by employing a continuous-time stochastic signaling game framework. In our framework, an adversary plays a stopping game, interacting with the system (having imperfect information about the type of an adversary, i.e., honest or malicious) to obtain explanation variance information and computing an optimal threshold to determine the membership of a datapoint accurately. First, we propose a sound mathematical formulation to prove that such an optimal threshold exists, which can be used to launch MIA. Then, we characterize the conditions under which a unique Markov perfect equilibrium (or steady state) exists in this dynamic system. By means of a comprehensive set of simulations of the proposed game model, we assess different factors that can impact the capability of an adversary to launch MIA in such repeated interaction settings.

==> abstract_old.tex <==

Model explanations, such as gradient-based explanations, improve the transparency of black-box machine learning (ML) models and their decisions, but they can also be exploited to carry out privacy threats such as membership inference attacks (MIA). This paper studies a variation of MIAs, referred to as explanation-based threshold attacks, where an adversary attempts to infer the membership of a set of data points from the computed variances of the gradient-based explanations by repeatedly interacting with the system (target ML model and its associated explanation method).
%The adversary's goal is to utilize historical (explanation) information to determine an appropriate explanation variance threshold that can be employed to determine the (training) membership of a set of data points. 
We model these strategic repeated interactions between an adversary and the system by means of a continuous-time stochastic Signaling game framework. In this game, on the one hand, 
%There is a strategic interplay here between the adversary and the model that needs to be formally modeled in order to understand the feasibility conditions for such attacks.
the adversary must strategically decide when to stop querying the target model in order to reach the target variance,
%\mj{can we replace ``assigned target" with something else? ``target variance"?}
all without being detected. On the other hand, the system which has imperfect information about the type of end-user (malicious or honest) it is interacting with, 
%(i.e., it could be interacting with an honest user or a malicious adversary) 
must strategically decide based on its Bayesian belief (about the end-user's type), how much information (in the form of noisy explanations) it should share, and when to stop sharing to prevent such MIAs. 
%This paper models this strategic interaction by means of a continuous-time stochastic Signaling game framework, and 
This paper characterizes the conditions under which a unique Markov perfect equilibrium (or steady state) exists in this setup. By means of extensive numerical simulations, the above game model is analyzed for four gradient-based explanation methods, namely, Integrated Gradients, Gradient*Input, LRP, and Guided Backpropagation. Additional experiments on five popular datasets (Purchase, Texas, CIFAR-10, CIFAR-100, and the Adult census) are also conducted to analyze the game's evolution and the adversary's MIA accuracy using the computed explanation variance threshold.



%computed through the game analysis.

%%%%%%%Kavita Old
%We study explanation-based threshold attacks in which an adversary can infer the membership of the data points by utilizing explanation variances that she/he computes for the explanations received from the \texttt{system} (comprising of a machine learning model and the associated explanation method). An adversary is an \texttt{end-user} who can query the \texttt{system} to get the query's label and its explanation. The goal of an adversary is to utilize historical (explanation) information to attain the \emph{explanation variance threshold} that he/she can efficiently employ to determine the membership of the data points.
%Thus, he/she must strategically decide when to stop querying the \texttt{system} to reach the assigned target, all without being detected by the \texttt{system}. We have assumed a \texttt{system}, which has imperfect information about the activity or the type of the \texttt{end-user} (honest or malicious), it is interacting with. Thus, it forms a Bayesian prior, which encodes such activity or the type of the \texttt{end-user}. The \texttt{system} must strategically decide how much information (in the form of noisy explanations) it should share with the \texttt{end-user} and when to stop sharing, based on its Bayesian belief only to prevent such attacks. We model this problem as a continuous-time stochastic Signaling game framework and characterize the conditions under which a unique Markov perfect equilibrium exists. Following that, we perform numerical simulations to analyze the game evolution for four gradient-based explanation methods, namely,  \emph{Integrated Gradients}, \emph{Gradient*Input}, \emph{$\epsilon$-LRP}, and \emph{Guided Backpropagation}. We also conduct experiments for five popular datasets, namely, Purchase, Texas, CIFAR-10, CIFAR-100, and the Adult census dataset; we analyze the game's evolution and the Membership Inference Attack accuracy of the adversary with respect to the explanation variance threshold computed through the game analysis.

==> exp_setup_eval.tex <==

\section{Experimental Setup}
\label{sec:setup}
We employ the \emph{Captum} \cite{kokhlikyan2020captum} framework to generate four different types of explanations, namely, Integrated Gradients, Gradient*Input, LRP, and Guided Backpropagation, and the \emph{PyTorch} framework to conduct the training and attack-related experiments. As Integrated Gradients, LRP, and Guided Backpropagation are nothing but improved versions of Gradient*Input, we use the Gradient*Input explanation method as the baseline (to compare the results of the other explanation methods). As mentioned in \cite{shokri2021privacy}, high explanation variance values at any datapoint $\overrightarrow{x}$ indicates that $\overrightarrow{x}$ was not used for training the model, %the model is uncertain about the prediction of $\overrightarrow{x}$ paving the way towards a potential attack by an adversary.
thus, our objective in all the experiments is to analyze and compute the impact of different settings (factors) that can impact the capability of an adversary to launch MIA. We assume that when the game ends, both the \texttt{system} and the \texttt{end-user} will have access to their optimal strategies, thus the optimal explanation variance threshold ($u_{th}$ for the \texttt{system} and $l_{th}$ for the \texttt{end-user}). Hence, an adversary can use its optimal strategy and optimal threshold to conduct MIA, or a \texttt{system} can use its optimal strategy and optimal threshold to protect against MIA. As a result, we focus on 
two evaluation objectives in our experiments: (i) \emph{game evolution}, and (ii) \emph{MIA accuracy}. For the game evolution, we compute the mean and the standard deviation of the variance of the explanations generated for the test datapoints (for all the datasets mentioned below) to simulate and generate the future explanation variances for $t=100$ stages, according to the expression:
\begin{equation}
    EX_{t}^{v} = EX_{0}^{v} * e ^{\left((\mu-\frac{1}{2}\sigma^{2}) + \sigma W_{t}\right)} \label{eqn:gbm}
\end{equation}
%We will first use the \emph{Gradient*Input} to generate explanations and examine the existence of MPE in each of the dataset outlined below.
The above equation is the solution to the GBM (\ref{subsec:setup}) of $EX_{t}^{v}$, derived using the \textit{it$\hat o$'s} calculus \cite{dixit2012investment}. 
%$\mu$ is the constant \emph{drift} and $\sigma > 0$ is the constant \emph{volatility} of the variance process $EX_{t}^{v}$, and
$\mu$ and $\sigma > 0$ are computed using the variance generated for the test datapoints for each of the dataset. 
%$EX_{0}^{v}$ is the initial explanation variance computed at $t=0$.
In our experiments, we take $EX_{0}^{v}$ as the last index value of the test data points' generated explanation variance, as we use this initial value to generate future explanations. 
Using the obtained optimal strategies and thresholds, we compute the attack accuracy in terms of the attacker's success rate in launching the MIA or the accuracy of the \texttt{system} in preventing MIA. 
%\mj{check-I edited this sentence}.
%After the analysis of the game or when the game ends, both the \texttt{system} and the \texttt{end-user} will have access to their optimal strategies, thus the optimal explanation variance threshold ($u_{th}$ for the \texttt{system} and $l_{th}$ for the \texttt{end-user}). 


Below we provide the configurations of the different datasets used in the game evaluation and the metric we employ to measure the accuracy of the attacks. 

\noindent
\textbf{Datasets. }We use five popular benchmark datasets on which we perform our game analysis and attack accuracy evaluations: Purchase and Texas datasets \cite{nasr2018machine}, CIFAR-10 and CIFAR-100 \cite{sablayrolles2019white}, and the Adult Census dataset \cite{Dua:2019}. To ease the comparison, the setup and Neural Network (NN) architectures are aligned with existing work on explanation-based threshold attacks \cite{shokri2021privacy}.

\emph{Purchase:} This dataset is downloaded from Kaggle's ``Acquire Valued Shoppers Challenge" \cite{shoppers}. The challenge aims to predict customers that will make a repeat purchase. The dataset has $197,324$ customer records, with each record having $600$ binary features. The prediction task is to assign each customer to one of the $100$ labels. We use the same NN architecture used by Shokri et al. \cite{shokri2021privacy}, a four-layer fully connected neural network with \textit{tanh} activations and layer sizes equal to $1024$, $512$, $256$ and $100$. We use \textit{Adagrad} optimizer with a learning rate of $0.01$ and a learning rate decay of $10^{-7}$ to train the model for $50$ epochs.

\emph{Texas:} This dataset contains patient discharge records from Texas hospitals \cite{texas}, spanning years 2006 through 2009. It has been used to predict the primary procedures of a patient based on other attributes such as hospital id, gender, length of the stay, diagnosis, etc. This dataset is filtered to incorporate only 100 classes (procedures) and has 67,330 records. The features are transformed to include only binary values, such that each record has 6,170 features. We use a five-layer fully connected NN architecture with \textit{tanh} activations and layer sizes of 2048, 1024, 512, 256 and 100. We employ the \textit{Adagrad} optimizer with a learning rate of 0.01 and a learning rate decay of $10^{-7}$ to train the model for 50 epochs.

\emph{CIFAR-10 and CIFAR-100:} CIFAR-10 and CIFAR-100 are the benchmark datasets for image classification tasks. Each dataset consists of 50K training and 10K test images. As NN architecture, we designed two convolutional layers with max-pooling and two dense layers, all with \textit{tanh} activations for CIFAR-10 and using Alexnet \cite{krizhevsky2012imagenet} for CIFAR-100. We train the model for 50 epochs with learning rates of 0.001 and 0.0001 for CIFAR-10 and CIFAR-100, respectively. In both cases, we use \textit{Adam} optimizer to update the parameters of the model.

\emph{Adult:} This dataset is downloaded from the 1994 US Census database \cite{Dua:2019}. It has been used to predict whether a person's yearly income is above 50,000 USD or not. It has 48,842 records and has a total of 14 features, including categorical and numeric features. After transforming categorical features into binary features, each data point resulted in having 104 features. A dataset of 5,000 data points is sampled from the original dataset because of the large size, containing 2,500 training data points and 2,500 testing data points. We use a five-layer fully-connected NN architecture with \textit{tanh} activations and layer sizes equal to 20, 20, 20, 20 and 1. We use an \textit{Adagrad} optimizer with a learning rate of 0.01 and a learning rate decay of $10^{-7}$ to train the model for 50 epochs.


\begin{table}[t]
\centering
%\caption{Configuration of the datasets utilized in the analysis of the game.}
\caption{Dataset Configurations.}
\begin{tabular}{| c | c |c | c | c |} 
 \hline
\textbf{Datasets} & \textbf{Points} & $\#$\textbf{Features} & \textbf{Type} & $\#$\textbf{Classes} \\  \hline
 Purchase             & 197,324           & 600 					  & Binary            & 100  \\ \hline
 Texas 			  & 67,330 		  & 6,170 				  & Binary            & 100 \\ \hline
 CIFAR-100   	  & 60,000    	  & 3,072				  & Image 		 & 100 \\ \hline
 CIFAR-10      	  & 60,000       	  & 3,072 				  & Image            & 2 \\ \hline
  Adult			  & 48,842		  & 24					  & Mixed 		 & 2  \\ \hline
\end{tabular}
\label{tab:datasets}\vspace{-0.2cm}
\end{table}



\noindent
\textbf{Evaluation metric. }We compute \textit{True Positive Rate (TPR)} metric to estimate the accuracy (or sensitivity) of the explanation-based threshold attack after the game has ended and each player has formulated the best response strategy concerning the other player. \textit{TPR} specifies how accurately an attacker can infer the membership of the data points.
%After the game analysis, as mentioned earlier, we assume that both the \texttt{system} and the \texttt{end-user} will have access to their optimal strategies, i.e., will have access to the explanation variance upper thresholds $u_{th}$ and $l_{th}$, respectively.
As we already know the membership of the training data points for each of the datasets, we use them to compute the TPR as follows: first, we compute the explanation variance of the training set, and then, we compare the obtained explanation variance with the \texttt{system}'s $u_{th}$ to determine how many points explanation variance lies below $u_{th}$ as mentioned in Section \ref{subsec:mia}.
%\mj{This is NOT CLEAR AT ALL. Let's discuss this!}. 
The total number of training data points correctly inferred as training points are called True Positives ($TP$), while the number of training members discerned as non-training members are called False Negatives ($FN$). Thus, $TPR = \frac{TP}{TP+FN}$. 




\section{Evaluation}
\label{sec:eval}

In this section, we present experimental analyses of our game model, wherein we compute the impact of different settings on two objectives: (i) the game or equilibrium evolution to obtain optimal strategies and (ii) attack accuracy, i.e., TPR. 
We begin by analyzing the impact of the \emph{Gradient*Input} explanations (baseline) on the game equilibrium and attack accuracy for all the considered datasets, 
%mentioned in Section \ref{sec:setup} 
and then compare it with the results obtained for the other explanation methods. After that, we also analyze the influence of other factors (e.g., input dimension and overfitting) on the attack accuracy. 

\subsection{Impact of Different Attack Information Sources}
%In this section, we first analyze the game's evolution for the different datasets mentioned in the previous section for the baseline setting. Then, we compute the attack accuracy of the launched explanation-based threshold attacks (Section \ref{subsec:mia}) by determining the $TPR$. Lastly, we perform the same analysis for other explanation methods and compare the obtained results with the results of the baseline setting.
%In order to simulate the variance of the explanations as GBM, we first compute a list of the explanation variances as mentioned in Section \ref{sec:setup} for the test data points for each dataset. Then, we estimate the mean and standard deviation of explanations variance generated for the output labels and use that to 
As mentioned in Section \ref{sec:setup}, for each dataset, we first sample a series of (future) explanations by employing GBM (using Equation \ref{eqn:gbm}). 
%Noise to be added to the explanations variance provided by the \texttt{system} to the \texttt{end-user} is sampled from a Normal distribution with the same mean and standard deviation of the generated explanations variances. 
The sampled noise is added to the generated explanations variance based on the computed belief at that time (using Bayes' rule in Section \ref{subsec:setup}), such that larger the belief that the \texttt{end-user} is honest, the smaller the noise value added to the explanation, and vice-versa. 
%Game model parameters that we chose in our numerical simulations for all explanation techniques are outlined in Table \ref{fig:sys_parameters} in the Appendix.
Then, we compute different functional paths for the \texttt{system} and the \texttt{end-user} defined in Section \ref{subsec:eqdesc} using the closed form representation detailed in Section \ref{subsec:ana;ytical}, i.e., we compute $U(\pi_{t})$, $L^{+}(\pi_{t})$,  $L^{-}(\pi_{t})$ and  $L(\pi_{t})$ functions. 
% assumed in figure \ref{fig:sys_parameters} (in Appendix \ref{subsec:gp}) for each of the explanation method.  
The termination payoff, $\lambda(ex^{v}_{e_{u}},\pi_{t})$ (defined in \ref{subsec:ctbw}), which is used to write the boundary conditions in the computation of $L^{+}(\pi_{t})$,  $L^{-}(\pi_{t})$ and  $L(\pi_{t})$ (Lemma \ref{lemma:lplus} and Lemma \ref{lemma:lminus}, and Theorem \ref{thm:optL}) is assumed to be:
\begin{equation}
\lambda(ex^{v}_{e_{u}},\pi_{t}) = \frac{0.8 \times ex^{v}_{e_{u}} \times log({\pi_{t} \times 2}) + \pi_{t} \times ex^{v}_{e_{u}}}{b} \nonumber
\end{equation}
where, $ex^{v}_{e_{u}}$ is the value of any \texttt{end-user}'s functional path (considered for the specific computation) at time $t$, and $b$ is the model parameter set differently for each explanation method. The parameters to compute $\lambda(ex^{v}_{e_{u}},\pi_{t})$ are empirically chosen based on their suitability to each of the four explanation methods considered in the paper. Based on our numerical simulations, below are some important observations we make for each dataset, both in the baseline setting (i.e., for the \emph{Gradient*Input} method) and the other three gradient-based explanation techniques.

\begin{figure}[!ht]
     \centering
     \iffalse
      \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/cifar-10/ex_toeu_g_vs_tem_g_copy.pdf}
         \caption{CIFAR-10}
         \label{fig:cifar10_exge_vs_exgi}
     \end{subfigure}
     \fi
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/cifar-10/diff_variance_eu.pdf}
         \caption{CIFAR-10}
         \label{fig:cifar10_diff_var_eu}
     \end{subfigure}
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/cifar-10/diff_variance_system.pdf}
         \caption{CIFAR-10}
         \label{fig:cifar10_diff_var_system}
     \end{subfigure}
     \iffalse
     \centering
      \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/cifar-100/ex_toeu_g_vs_tem_g_copy.pdf}
         \caption{CIFAR-100}
         \label{fig:cifar100_exge_vs_exgi}
     \end{subfigure}
     \fi
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/cifar-100/diff_variance_eu.pdf}
         \caption{CIFAR-100}
         \label{fig:cifar100_diff_var_eu}
     \end{subfigure}
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/cifar-100/diff_variance_system.pdf}
         \caption{CIFAR-100}
         \label{fig:cifar100_diff_var_system}
     \end{subfigure}
    \iffalse
     %\centering
      \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Adult/ex_toeu_g_vs_tem_g_copy.pdf}
         \caption{Adult}
         \label{fig:adult_exge_vs_exgi}
     \end{subfigure}
     \fi
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Adult/diff_variance_eu.pdf}
         \caption{Adult}
         \label{fig:adult_diff_var_eu}
     \end{subfigure}
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Adult/diff_variance_system.pdf}
         \caption{Adult}
         \label{fig:adult_diff_var_system}
     \end{subfigure}
     \iffalse
      \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Purchase/ex_toeu_g_vs_tem_g_copy.pdf}
         \caption{Purchase}
         \label{fig:purchase_exge_vs_exgi}
     \end{subfigure}
     \fi
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Purchase/diff_variance_eu.pdf}
         \caption{Purchase}
         \label{fig:purchase_diff_var_eu}
     \end{subfigure}
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Purchase/diff_variance_system.pdf}
         \caption{Purchase}
         \label{fig:purchase_diff_var_system}
     \end{subfigure}
     \iffalse
      \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Texas/ex_toeu_g_vs_tem_g_copy.pdf}
         \caption{Texas}
         \label{fig:texas_exge_vs_exgi}
     \end{subfigure}
     \fi
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Texas/diff_variance_eu.pdf}
         \caption{Texas}
         \label{fig:texas_diff_var_eu}
     \end{subfigure}
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Texas/diff_variance_system.pdf}
         \caption{Texas}
         \label{fig:texas_diff_var_system}
     \end{subfigure}
        \caption{Different functional paths for the different datasets. (a), (c), (e), (g), and (i) represents the optimal functional paths for the \texttt{end-user}. (b), (d), (f), (h), and (j) represents the optimal functional paths for the \texttt{system}.}
        \label{fig:baseline_game}\vspace{-0.3cm} 
\end{figure}


\noindent
\textbf{Game Evolution in the Baseline Setting: }
Varying game evolution is realized for different datasets, as shown in Figure \ref{fig:baseline_game}. Below we analyze in detail the optimal paths obtained for each of the dataset. 
\begin{itemize}[leftmargin=*]
\item From the plots of the optimal functional path $U(\pi_{t})$ of the \texttt{system} for each of the dataset, as shown in Figures \ref{fig:cifar10_diff_var_system}, \ref{fig:cifar100_diff_var_system}, \ref{fig:adult_diff_var_system}, \ref{fig:purchase_diff_var_system}, and \ref{fig:texas_diff_var_system}, we can observe that as $\pi_{t} \rightarrow 1$, $U(\pi_{t})$ starts decreasing. This is because, as the \texttt{system}'s belief about the type of \texttt{end-user} approaches $1$, both the variance of the explanation generated by the system and the variance of the noisy explanation given to the \texttt{end-user} approach $u_{th}$ and $l_{th}$, respectively. After a certain point, i.e., when $ex^{v}_{s_{y}} > U(\pi_{t})$, the \texttt{system} will block the \texttt{end-user}, which confirms to our intuition.
%%when $ex_{ge}(\pi_{t}) > U(\pi_{t})$, the \texttt{system} will block the \texttt{end-user}.
\item From the optimal functional paths $L^{+}(\pi_{t})$,  $L^{-}(\pi_{t})$ and  $L(\pi_{t})$ of the \texttt{end-user} for each of the dataset, as shown in Figures \ref{fig:cifar10_diff_var_eu}, \ref{fig:cifar100_diff_var_eu}, \ref{fig:adult_diff_var_eu}, \ref{fig:purchase_diff_var_eu}, and \ref{fig:texas_diff_var_eu}, we can observe that as $ \pi_{t} \rightarrow 1$,  $L^{+}(\pi_{t})$,  $L^{-}(\pi_{t})$ and  $L(\pi_{t})$ approach the threshold $l_{th}$. As discussed in \ref{subsec:eqdesc}, as $ \pi_{t} \rightarrow 1$ and the variance of the explanation given to the \texttt{end-user} starts to approache the variance threshold, it means a malicious \texttt{end-user} is trying to compromise the \texttt{system}. Thus, if the \texttt{system} doesn't block the \texttt{end-user} at the right time (or doesn't have knowledge about optimal $U(\pi)$), then the \texttt{end-user} can easily compromise the \texttt{system}. 

\item Earlier we showed that a unique MPE exists when $L^{+}(\pi_{t})$ and $L^{-}(\pi_{t})$ begin to converge as $\pi_{t} \rightarrow 1$. 
%%So, we try to find out the first intersection point (root) of $L^{+}(\pi_{t})$ and $L^{-}(\pi_{t})$ as the unique MPE. 
This is also visible from our results as shown in Figure \ref{fig:baseline_game}, where we can observe that as $ \pi_{t} \rightarrow 1$, $L^{+}(\pi_{t})$ and  $L^{-}(\pi_{t})$ starts to converge. However, for the CIFAR-10 dataset, one can observe that the curves $L^{+}(\pi_{t})$ and  $L^{-}(\pi_{t})$ doesn't converge as $ \pi_{t} \rightarrow 1$. Thus, an MPE doesn't exist in the case of CIFAR-10 dataset. The intuition behind this observation is that the fluctuations (or variance) of the explanation variance computed for the CIFAR-10 is high, making it difficult for them to converge to a single point. 
%When curves $L^{+}(\pi_{t})$ and $L^{-}(\pi_{t})$ converge, $L(\pi_{t}) =L^{+}(\pi_{t})=L^{-}(\pi_{t})$ or we have reached an equilibrium. 
Finally, if the \texttt{system} doesn't block the \texttt{end-user} before the threshold $l_{th}$ or $u_{th}$ is reached, then we say a unique MPE exists in the game.  
\end{itemize}





\noindent
\textbf{Attack Accuracy in the Baseline Setting: }After obtaining the optimal strategies, we use the range of the training data points of each dataset to determine how many data point variances lie below the computed threshold $u_{th}$ to determine their membership. As shown in Figure \ref{fig:acc_basemethod}, the attack accuracy for all the datasets except CIFAR-10 is more than 50\%. This result aligns with the observed game equilibrium analysis. Hence, the fluctuations in explanation variance make it difficult for an adversary to reach the target threshold, in consequence, to launch MIAs. From these obtained results, one can easily observe that the explanations provide a new opportunity or an attack vector to an adversary actively trying to compromise the \texttt{system}. In other words, our results are clear indicators that an adversary can repeatedly interact with the \texttt{system} to compute the explanation variance threshold and successfully launch membership inference attacks against the \texttt{system}.



\noindent
\textbf{Results for other Explanation Techniques: }
We also analyzed the game for the three other explanation methods considered in this paper. We do not plot the game evolution results in this setting as the plots follow a very similar trend as seen in Figure \ref{fig:baseline_game}, i.e., game equilibrium was achieved for all the datasets except for the CIFAR-10. We uses the same setting as the baseline setting (mentioned above) to compute attack accuracy for these three explanation methods.
%We again used training data points for each of the datasets: Texas, Purchase, CIFAR-10, and Adult, to compute the attack accuracy of an attacker.
%Thus, for the prediction label of any training data points, if the computed explanation variance is below $u_{th}$, then an attacker successfully determines the training membership of that data point.
We obtained each dataset's attack accuracy as shown in Figure \ref{fig:acc_othermethod}. %One can observe from this plot that 
For the Texas and Purchase datasets, 100\% accuracy was achieved, i.e., an attacker effectively determines the membership of all the data points used for training the model. However, for the CIFAR-10, the attack accuracy was below 50\%, and for the Adult dataset, attack accuracy was above 50\% only for the LRP explanation method. The reason is again the high fluctuations in the computed variance for the CIFAR-10 dataset (slightly less for the Adult dataset), thus making it difficult for an adversary to determine the membership of the data points in those datasets. These results clearly indicate that, for different explanation methods, 
%\mj{why sources? can we say ``methods"?},
an adversary's capability to launch MIA attacks will vary and may depend on the variance of the explanations.
%\mj{check this para - I made edits}
%\am{this paragraphs is poorly written compared to rest of the paper. i can improve this after kavita is done with MJ's comments}.

\begin{figure}[!ht]
     \centering

      \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\textwidth,trim=0.2cm 0.4cm 0.2cm 0]{Figures/acc_train_base.pdf}
         \caption{}
         \label{fig:acc_basemethod}
     \end{subfigure}
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\textwidth, trim=0.2cm 0.4cm 0.2cm 0]{Figures/acc_train_diff.pdf}
         \caption{}
         \label{fig:acc_othermethod}
     \end{subfigure}\vspace{-0.15cm}
        \caption{$TPR$ rates for the optimal strategy obtained by the \texttt{system} and the \texttt{end-user}: a) $\emph{Gradient*Input}$ method and b) Other explanation methods.}
        \label{fig:base_acc}\vspace{-0.3cm}
\end{figure}
\iffalse
\begin{figure*}[H]
     \centering

      \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth,trim=0.3cm 0.4cm 0.3cm 0]{Figures/k_100/belief.pdf}
         \caption{}
         \label{fig:belief_100_old}
     \end{subfigure}
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth,trim=0.3cm 0.4cm 0.3cm 0]{Figures/k_100/belief_NM.pdf}
         \caption{}
         \label{fig:belief_100_new}
     \end{subfigure}
    \begin{subfigure}[b]{0.2\textwidth}
\centering
\includegraphics[width=\linewidth,trim=0.3cm 0.4cm 0.3cm 0]{Figures/k_100/ex_toeu_g_vs_tem_g_copy.pdf}
\caption{}
\label{fig:ex_toeu_vs_exgi}
\end{subfigure}\vspace{-0.15cm}
     
        \caption{Belief ($\pi_{t}$) evolution of the \texttt{system} for the model having $k=100$ classes and data points having $n_{f} = 100$ features.}
        \label{fig:base_acc}\vspace{-0.3cm}
\end{figure*}
\fi

%\vspace{-0.1cm}
\subsection{Analysis of other Relevant Factors}
\label{subsec:other}
In this section, we analyze the influence of other factors such as input dimension, underfitting, and overfitting, which can impact the equilibrium evolution, and thus the accuracy of the explanation-based threshold attacks. 
For this, we analyze the game's evolution on synthetic datasets and the extent to which an adversary can exploit model gradient information to conduct membership inference attacks. Using artificially generated datasets helps us identify the important factors that can facilitate information leaks.

\begin{itemize}[leftmargin=*]
\item \textbf{Impact of Input dimension. }
First, we analyze the impact of the input dimension of the data points on the game evolution. To generate datasets, we used the Sklearn make classification module \cite{scikit-learn}. The number of classes is set to either 2 or 100, while the number of features will vary in range $t_{f} \in [10, 100, 1000, 6000]$. For each setting, we sample 20,000 points and split them evenly into training and test set. Second, for each value $t_{f}$ and for each class, we employ two models to train from this data, namely, model $A$ and model $B$. Model $A$ is chosen to have less
%\am{fewer?}
layers (or depth) than model $B$; to compare the effect of the complexity of the models on the game evolution and attack accuracy. Model $A$ is a fully connected NN with two hidden layers
%\am{composed of}
fifty nodes each, the \textit{tanh} activation function between the layers, and \textit{softmax} as the final activation. The network is trained using \textit{Adagrad} with a learning rate of 0.01 and a learning rate decay of $10^{-7}$ for 50 epochs. Model $B$ is a five-layer fully connected NN with \textit{tanh} activations. The layer sizes are chosen as 2048, 1024, 512, 256 and 100. We use the \textit{Adagrad} optimizer with a learning rate of 0.01 and a learning rate decay of $10^{-7}$ to train the model for 50 epochs. Next, we demonstrate the effect of these models on our experiment's two main objectives. 
%\am{the two objectives are commented out earlier}.
%\K{Do you want me to write it down here?}

\begin{itemize}
    \item \textbf{Effect of Model $A$ on Game Evolution and Attack Accuracy. }For $k=2$ classes, we observe a similar trend in the game evolution as shown in Figure \ref{fig:baseline_game} for each of the features $t_{f} \in [10, 100, 1000, 6000]$. However, for $k=100$ classes, we observed that the belief $\pi_{t}$ of the \texttt{system} about the type of the \texttt{end-user} is always set to $1$ as shown in Figure \ref{fig:belief_old}. As a consequence, the variance of the explanations generated is equivalent to the variance of the explanations given, as shown in Figure \ref{fig:ex_toeu_vs_exgi}. Hence, the game didn't evolve as the \texttt{system} gave the same explanation to the \texttt{end-user}. The reason is because of underfitting. Model $A$ simply does not have enough depth (in terms of the number of layers) to accurately classify 100 classes. Thus, it was not able to accurately classify $100$ classes. Moreover, the loss of model $A$ was approximated to be around $5.74$ for all the features considered, which is not accurate. Hence, the model $A$ gives erroneous results for model predictions. In consequence, it impacts the two objectives of the experiments. 
    %\mj{instead of ``good" can we use the word ``accurate"?}.
\begin{figure}[H]
     \centering
     \vspace{-0.5cm}
      \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\textwidth, trim=0.2cm 0.4cm 0.2cm 0]{Figures/k_100/belief.pdf}
         \caption{}
         \label{fig:belief_old}
     \end{subfigure}
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\textwidth, trim=0.2cm 0.4cm 0.2cm 0]{Figures/k_100/ex_toeu_g_vs_tem_g_copy.pdf}
         \caption{}
         \label{fig:ex_toeu_vs_exgi}
     \end{subfigure}\vspace{-0.3cm}
        \caption{Explanation variance generated vs. explanation variance given when $\pi_{t}=1$.}
    \label{fig:belief_pattern}\vspace{-0.3cm}
\end{figure} 
    \item \textbf{Effect of Model $B$ on Game Evolution and Attack Accuracy.} In this case, we considered model $B$ of higher complexity (more layers compared to model $A$) that led to different results compared to model $A$. For $k=2$ classes and $n_f = 10$, we did not observe any game evolution, because for the test data points explanation variance we got $\sigma > \mu$ and $\sigma > 1$. Consequently, the values of the computed future variance of the explanation, using Equation \ref{eqn:gbm}, were zero. However, for $t_{f} \in [100, 1000, 6000]$, we observed the game equilibrium and computed the attack accuracy by sampling from the training data points, as shown in Figure \ref{fig:k_2_nm}. For $t_{f}=1000$, an attack accuracy greater than 50\% was observed, however, for $t_{f}=100$ and $t_{f}=6000$, an attack accuracy less than 50\% was observed. For $k=100$ classes, we did not observe any equilibrium for any of the features $t_f$. Therefore, based on the last index value of the explanation variance simulated (i.e. at $t=100$), we computed the threshold $u_{th}$ and accordingly determined the attack accuracy for each of the features as shown in Figure \ref{fig:k_100_nm}. In this setting, the loss of the model $B$ was approximated to be around $0.8$ for all the features considered. 
\end{itemize}

The results obtained for models $A$ and $B$ indicate that the choice of the model used for the classification task on hand also affects the game evolution, and thus, an adversary's capability to launch MIA attacks against the \texttt{system}.


\iffalse
\begin{figure}[ht]
\centering
\includegraphics[width=0.75\linewidth]{Figures/k_100/ex_toeu_g_vs_tem_g_copy.pdf}
\caption{Explanation variance generated vs. explanation variance given when $\pi_{t}=1$.}
\label{fig:ex_toeu_vs_exgi}
\end{figure}
\fi

\begin{figure}[H]
     \centering

      \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\textwidth, trim=0.4cm 0.4cm 0.2cm 0]{Figures/k_2/k_2_nm.pdf}
         \caption{$k=2$.}
         \label{fig:k_2_nm}
     \end{subfigure}
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\textwidth, trim=0.4cm 0.4cm 0.2cm 0]{Figures/k_100/k_100_nm.pdf}
         \caption{$k=100$.}
         \label{fig:k_100_nm}
     \end{subfigure}\vspace{-0.1cm}
        \caption{MIA accuracy for different features $n_f$ for model $B$.}
        \label{fig:k_nm}\vspace{-0.3cm}
\end{figure}




\item
\textbf{Impact of  Overfitting.} 
As detailed in \cite{yeom2018privacy}, overfitting can significantly increase the accuracy of the membership inference attacks. Thus, to see its effect on the game evolution and attack accuracy in our setup, we varied the number of epochs of the training process. We chose Purchase, Texas, and Adult datasets for this setting. As mentioned in Section \ref{sec:setup}, the models for these datasets are trained for 50 epochs; thus, to observe the impact of the number of epochs, we trained the models of each dataset for epochs in
%\mj{this sentence is not clear. What do you mean conducted experiments for epochs? Do you mean you trained for these many epochs?}
\{30, 50, 60\}.
%\mj{I don't think you should use square brackets here. Use paranthesis.e.g., \{30, 50, 60\}}.
The results are shown in Figure \ref{fig:epoch_acc}. We observed that overfitting only increased the attack accuracy for the Adult dataset, while it remained the same for the Texas dataset and decreased for the Purchased dataset. The reason is that the game evolution, and thus the MIA accuracy, depends on multiple factors (mentioned above), hence, the number of training epochs will not singularly determine or impact the capability of an adversary to launch MIA, as presented in the different scenarios mentioned earlier. In other words, the above results show that overfitting does not necessarily increase the attack's accuracy.

\begin{figure}[H]
\centering
\includegraphics[width=0.65\linewidth]{Figures/epochs_acc.pdf}\vspace{-0.3cm}
\caption{MIA accuracy for different datasets trained for different epochs.}\vspace{-0.3cm}
\label{fig:epoch_acc}
\end{figure}

\end{itemize}










==> intro_old.tex <==
%\section{Introduction}
%\label{sec:Intro}
Machine learning (ML) models are currently employed by almost every major industry and service provider to make critical data-based decisions \cite{bhavsar2017machine, ahmad2018interpretable, ballestar2019predicting, dixon2020machine}. Due to the complex and black-box nature of these models, where model description is hidden behind millions of parameters and is unavailable to end-users, comprehending the underlying reasons/justifications behind model decisions is often extremely difficult, if not impossible. Consequently, there has been increased public and regulatory pressure to design and deploy automated model explanation techniques that provide a better understanding of the behavior and predictions of opaque ML models, effectively improving their transparency and reliability \cite{GoodmanFlaxman17aimag}. This has resulted in the availability of several novel model explanation techniques and toolkits, both from academia \cite{ribeiro2016should, lundberg2017unified, shrikumar2017learning, arras2017relevant, jacovi2018understanding, ancona2018towards} and industry \cite{GoogleMLInt, microsoftMLInt}. Simultaneously, 
%Although explanations provide additional information related to model decisions, thereby improving model transparency and reliability, 
explanations also expose an attack surface that can be exploited to either infer private model information \cite{shokri2021privacy} or launch adversarial attacks against the model \cite{ignatiev2019relating, slack2020fooling}.


Our focus here is in the former direction, specifically, on
%i.e., inference of private model information from released explanations, 
% Although there have been several efforts on designing attack mechanisms to infer private information in ML algorithms, there is 
one very fundamental adversarial attack called the \emph{membership inference attack} (or MIA) \cite{ShokriSSS17,LongBG2017,pmlr-v97-sablayrolles19a}, where an adversary attempts to determine whether a data-point belongs to the training dataset of a pre-trained blackbox ML model or not. In this work, we focus on \emph{explanation-based membership inference attacks}, where an adversary leverages model explanations to infer training dataset membership (of some target data point).

Recently, Shokri et al. \cite{shokri2021privacy} investigated the feasibility of explanation-based MIA attacks, where they showed that the variance of the backpropagation-based explanations, i.e., the variance of the influence vector across different features, can help determine training set membership. The authors attribute this connection between explanation vector variance and training set membership to how 
%backpropagation-based 
training algorithms behave upon convergence. During training, such learning algorithms minimize the loss function by pushing the decision boundary away from the training data points. Thus, the high variance of the explanation (or influence) vector for a particular data point may be indicative of it being close to the decision boundary, which is more common for data points outside the training set. Based on this observation, the authors in \cite{shokri2021privacy} proposed an \emph{explanation-based threshold attack} for membership inference, where a data point is considered a member (of the training set)
%the dataset used to train the target model)
if and only if the variance of the corresponding gradient-based explanation (vector) is less than or equal to some threshold. 

The most important requirement in such explanation-based threshold attacks is, \emph{how to obtain or compute such a variance threshold?} It is trivial to compute an \emph{optimal} threshold if the training set membership of the target dataset is known. Alternatively, if the adversary has access to some labeled data from the target distribution and has access to the training hyperparameters and model architecture, 
%it can be used to train shadow/reference models and 
the variance threshold can be computed by training shadow or reference models, as suggested by Shokri et al. \cite{shokri2021privacy}. 
%However, the latter attack assumes that the adversary has access to the training hyperparameters and model architecture, in order to effectively train the shadow/reference models. 
This results in the following important question: \emph{how to carry out or accomplish such an explanation-based threshold attack, if an adversary does not have any knowledge of the model and it's training process?}
%when the above two assumptions do not hold, i.e, if the training set membership of the target dataset is unavailable and the training hyper parameters and model architecture are not known to train shadow models?}

One strategy for an adversary to accomplish this, assuming that he/she has access to some labeled data from the target distribution and that the pre-trained target model is continuously available as a black box, is to repeatedly interact with the target model (which outputs the prediction label and related backpropagation- or gradient-based explanation) in order to compute the explanation variance threshold. Once a sufficiently stable variance threshold is reached (or computed), it can be used (by the adversary) to determine the membership of any data point thereafter. We focus on this explanation-based threshold attack strategy in this work. Despite its simplicity, such a repeated interaction strategy raises several significant questions: \emph{how long should the adversary interact with the target model? can the target model detect such malicious interactions in a timely fashion to prevent membership inference?, and how can the target model strategically serve both honest and malicious users in such a setting?}

{\color{red}{Authors in \cite{patel2022model} designed differential private model explanations, which locally approximate the model around the point of interest, with the aim to prevent malicious users to extract private training data. However, such a defense lacks the study against a strategic adversary who can repeatedly interact with the \texttt{system} to infer private membership training data.}} Intuitively, the length and pattern of such repeated interactions should affect the amount of private information leaked by the model. However, currently, a proper understanding of this phenomenon is lacking, especially in the presence of a strategic adversary who wants to minimize the attack path (and cost) toward compromising model privacy and a strategic system that wants to prevent this without complete knowledge of the type of end-user (adversarial or non-adversarial) it is interacting with. {\color{red}{Also, how a \texttt{system} designs a defense against such a strategic adversary.}} We address this research gap by formally modeling the strategic interactions between such an adversary and an ML system through game theory, specifically a \emph{continuous-time stochastic Signaling Game} framework. 
%We address this research gap by formally modeling the strategic interactions between an adversary whose goal is to exploit gradient-based explanations for carrying out MIA (against a target black-box model) and the ML model who wishes to prevent such attacks while still providing reasonable gradient-based explanations to all users (including honest ones) by means of game theory, specifically a \emph{continuous-time stochastic Signaling Game} framework. 
%Such a formal understanding is the fundamental first step towards designing effective protection mechanisms against information leakage attacks from explanation techniques.
%
%In a similar domain, 

Game-theoretic approaches have been used in the research literature to model interactions with ML models, specifically to improve the robustness of ML models against adversarial examples. For instance, researchers have modeled adversarial classification games as zero sum games \cite{dekel2010learning} \cite{globerson2006nightmare}, non-zero sum games \cite{dritsoula2017game}, sequential Bayesian game \cite{zhou2014adversarial} \cite{grosshans2013bayesian}, sequential Stackelberg games \cite{bruckner2011stackelberg} \cite{alfeld2017explicit} and simultaneous game \cite{dalvi2004adversarial}. 
%In all these works, it has been assumed that an adversary attacks by either removing features from future input, or by changing values of future input or by mixing valid and adversarial input or by performing attacks on test dataset only. As mentioned earlier, we are assuming an adversary's objective to manipulate the query or the feature space for a series of queries, is to leverage the explanations, given by the \texttt{system}, to launch explanation-based threshold attacks. 
Contrary to these efforts, where an adversary's objective is to target the classification task of the ML model, our research effort focuses on the descriptive task of the ML model, i.e., explaining the model predictions.
%gradient-based explanation method (supporting the ). 
To the best of our knowledge, there has been no prior work that studies explanation-based threshold attacks for membership inference against a pre-trained blackbox model which provides repeated gradient-based explanations within a game-theoretic framework. We make the following specific contributions in this paper:
\begin{enumerate}[leftmargin=*]
\item We employ game theory to model the dynamics of explanation variance generated by a \texttt{system} (comprising of a ML model and the corresponding explanation technique) for predictions/labels related to queries sent by \texttt{end-users}. Specifically, we model the interactions between an \texttt{end-user} and the \texttt{system}, where variance of the explanations generated by the \texttt{system} evolve according to a \emph{stochastic differential equation (SDE)}, as a \emph{two-player continuous-time Signaling Game}. 
\item We then characterize the \emph{Markov Perfect Equilibrium (or MPE)} of the above stochastic game as a pair of two optimal functions:- $U(\pi)$ and $L(\pi)$, where $U(\pi)$ represents the optimal variance path for the explanations generated by the \texttt{system}, $L(\pi)$ represents the optimal variance path for the explanations given by the \texttt{system} to the \texttt{end-user} after adding some noise and $\pi$ represents the belief of the \texttt{system} about the type of \texttt{end-user}. 
\item We perform numerical simulations to analyze the game evolution for four gradient-based explanation methods, namely,  \emph{Integrated Gradients} \cite{sundararajan2017axiomatic}, \emph{Gradient*Input} \cite{shrikumar2016not}, \emph{LRP} \cite{bach2015pixel} and \emph{Guided Backpropagation} \cite{springenberg2014striving}. We also conduct experiments for five popular datasets, namely, Purchase, Texas, CIFAR-10, CIFAR-100, and the Adult census dataset, on which we analyze the game's evolution and the MIA attack accuracy of the attacker with respect to the explanation variance threshold computed through the game analysis. 
\end{enumerate}
%We employ game theory to model the dynamics of explanation variance generated by a \texttt{system} (comprising of a ML model and the corresponding explanation technique) for predictions/labels related to queries sent by \texttt{end-users}. Specifically, we model the interactions between an \texttt{end-user} and the \texttt{system}, where variance of the explanations generated by the \texttt{system} evolve according to a \emph{stochastic differential equation (SDE)}, as a \emph{two-player continuous-time Signaling Game}. 
%We then characterize the \emph{Markov Perfect Equilibrium (or MPE)} of the above stochastic game as a pair of two optimal functions:- $U(\pi)$ and $L(\pi)$, where $U(\pi)$ represents the optimal variance path for the explanations generated by the \texttt{system}, $L(\pi)$ represents the optimal variance path for the explanations given by the \texttt{system} to the \texttt{end-user} after adding some noise and $\pi$ represents the belief of the \texttt{system} about the type of \texttt{end-user}. 
%%The $L(\pi)$ value at any $\pi$ also gives the pooling interval of the two types of \texttt{end-users}.
%We then prove conditions for the existence and uniqueness of a MPE in the above game model.
%%using concepts from stochastic calculus and the study of ordinary differential equations. 
%Following that, we numerically analyze the existence of MPE and the optimal play (actions) of both the \texttt{system} and the \texttt{end-user} for four popular gradient-based explanation methods mentioned above.  


%Explanation-based threshold attack is defined as:
%
%For a given vector $\overrightarrow{v} \in \mathbb{R}^{n}$ of length $n$, the variance is computed as:
%
%$$Var(\overrightarrow{v}) = \sum_{i=1}^{n} (v_{i} - v_{m})^{2} \text{,} \quad \text{where} \, \, v_{m} = \frac{1}{n} \sum_{i=1}^{n} v_{i}$$
%
%Thus, for a defined threshold $v_{th}$ and an explanation vector, $H(\overrightarrow{x})$, computed for a query $\overrightarrow{x}$, an explanation-based threshold attack is given as:
%
%\[
%    Membership_{v_{th}}(\overrightarrow{x}) = 
%    \begin{cases}
%    \text{True},        & Var(H(\overrightarrow{x})) \geq v_{th} \\
%    \text{False},    & otherwise
%    \end{cases}
%\]
%
%
%Thus, a malicious \texttt{end-user} wants to reach the variance threshold ($v_{th}$) in order to infer the membership of the data-points. In \cite{shokri2021privacy}, authors have shown that the high variance of an explanation is an indicator for a point being close to a decision boundary. They have assumed that an adversary has obtained a set of data-points. $50\%$ of this set are members of the training set and this information is known to the adversary, which is used to compute the optimal variance threshold. Then, they have analyzed a single instance of an adversary conducting such attacks. However, in our work, we are trying to show how an adversary increasingly computes the variance to reach the variance threshold by repeatedly sending queries to the \texttt{system} to gain the explanatory information.

%<<<<<<<<<<<<<<<<<<<<<OLD INTRO - IGNORE FOR NOW>>>>>>>>>>>>>>>>>>>>>>
%Today, complex machine learning (ML) models are employed by almost every major sector of our economy for making critical data-based decisions \cite{bhavsar2017machine}, \cite{ahmad2018interpretable}, \cite{ballestar2019predicting}, \cite{dixon2020machine}.
%%, including, transportation \cite{bhavsar2017machine} \cite{jahangiri2015applying}, e-commerce \cite{ballestar2019predicting} \cite{guo2019securing}, healthcare \cite{mozaffari2014systematic} \cite{ahmad2018interpretable} and finance \cite{dixon2020machine} \cite{heaton2016deep},  with these models often tasked with making several important and high-stake data-based decisions. 
%%As each of these industries/sectors is growing, so is the number of services offered and the amount of data being collected, and thus the complexity of the machine learning models within the ecosystem. 
%One challenge while using complex ML models, such as, Deep Neural Networks (DNN), is that model description is hidden behind millions of parameters, making it impossible to comprehend model decisions.
%%we use machine
%%learning is that the comprehension of the task which machine learning
%%solves is hidden behind increasingly complex models. Millions of numbers are required to describe a deep neural network (DNN) entirely, and even then, there is no simple way to understand the model in its entirety. 
%%Moreover, the best performing models are often combinations of several models that cannot be interpreted, even if each single model within the ensemble could be interpreted. As a matter of fact, lately the focus has been purely on (model) prediction performance, which has effectively resulted in models that are less transparent and descriptive. 
%Consequently, there have been significant research efforts to design explanation techniques that provide a better understanding of the behavior and predictions by complex, pre-trained ML models, effectively improving their transparency and reliability \cite{shrikumar2017learning} \cite{lundberg2017unified} \cite{ribeiro2016should} \cite{arras2017relevant} \cite{jacovi2018understanding} \cite{ancona2018towards}. In this paper, our focus is on gradient-based explanation methods: Saliency Maps \cite{simonyan2014deep}, $\epsilon$- Layerwise Relevance Propagation ($\epsilon$-LRP) \cite{bach2015pixel}, Integrated Gradients \cite{sundararajan2017axiomatic} and Gradient*Input \cite{shrikumar2016not}. 
%
%One drawback of providing additional information as explanations is that it exposes an attack surface that can be exploited by an adversary to infer private model information \cite{shokri2021privacy} or launch adversarial attacks against the model \cite{ignatiev2019relating}\cite{slack2020fooling}. As mentioned earlier, our focus in this paper is on explanation-based threshold attacks, thus our work is motivated from \cite{shokri2021privacy}. Explanation-based threshold attack is defined as:
%
%For a given vector $\overrightarrow{v} \in \mathbb{R}^{n}$ of length $n$, the variance is computed as:
%
%$$Var(\overrightarrow{v}) = \sum_{i=1}^{n} (v_{i} - v_{m})^{2} \text{,} \quad \text{where} \, \, v_{m} = \frac{1}{n} \sum_{i=1}^{n} v_{i}$$
%
%Thus, for a defined threshold $v_{th}$ and an explanation vector, $H(\overrightarrow{x})$, computed for a query $\overrightarrow{x}$, an explanation-based threshold attack is given as:
%
%\[
%    Membership_{v_{th}}(\overrightarrow{x}) = 
%    \begin{cases}
%    \text{True},        & Var(H(\overrightarrow{x})) \geq v_{th} \\
%    \text{False},    & otherwise
%    \end{cases}
%\]
%
%
%Thus, a malicious \texttt{end-user} wants to reach the variance threshold ($v_{th}$) in order to infer the membership of the data-points. In \cite{shokri2021privacy}, authors have shown that the high variance of an explanation is an indicator for a point being close to a decision boundary. They have assumed that an adversary has obtained a set of data-points. $50\%$ of this set are members of the training set and this information is known to the adversary, which is used to compute the optimal variance threshold. Then, they have analyzed a single instance of an adversary conducting such attacks. However, in our work, we are trying to show how an adversary increasingly computes the variance to reach the variance threshold by repeatedly sending queries to the \texttt{system} to gain the explanatory information. We also have not made any assumption about the optimal variance threshold and is being computed using the required maths as shown in section \ref{sec:analysis}. This intuition is shown in figure \ref{fig:v_r} and figure \ref{fig:v_m}. Figure \ref{fig:v_r} represents the variance of the explanations generated when an honest or a random user repeatedly sends a query to the \texttt{system}. Since, an honest user is not trying to attack the \texttt{system}, the trend in variance is neither increasing or decreasing. However, the goal of the malicious \texttt{end-user} is to reach the variance threshold (to launch explanation-based threshold attacks), using the prior historical information, by repeatedly interacting with the \texttt{system}. This can be seen in the variance pattern in figure \ref{fig:v_m} and one can observe that the variance path is increasing. Hence, one key objective in this paper is to determine how much explanation (adding noise) a \texttt{system} should give to the malicious \texttt{end-user} to prevent such kinds of attacks based on it's Bayesian belief only. Also, because of the random, positive, and non-decreasing nature of the variance, we are assuming that the variance follows the Geometric Brownian Motion (GBM). 
%
%
%
%\begin{figure}
%     \centering
%	\begin{subfigure}{0.48\textwidth}
%	\centering
%  	\includegraphics[width=\textwidth]{Figures/variance_random.pdf}
%  	%\caption{Saliency Method.}
%	\vspace{-0.2in} \caption{}
%  	\label{fig:v_r}
%	\end{subfigure}
% 	\hfill
%  	\begin{subfigure}{0.48\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figures/variance_malicious.pdf}
%     %\caption{$\epsilon$-LRP.}
%	\vspace{-0.2in} \caption{}
%     \label{fig:v_m}
%	\end{subfigure}
%\caption{Plots for the variance of the explanations ($ex^{v}$) computed for the queries sent by the random or honest user and by the malicious user against time, $t$. a) Shows the random nature of the variance for the honest or random as he/she is not trying attack the system. b) Shows the increasing trend in variance for the malicious user as malicious user is exploring and exploiting the query space to reach a certain variance threshold.}
% \label{fig:exgie_given}
%\end{figure}
%
%%An adversary can either manipulate the input data-point \cite{dombrowski2019explanations}\cite{kindermans2019reliability} or manipulate the model \cite{slack2020fooling}\cite{ribeiro2016should}\cite{lundberg2017unified}\cite{dimanov2020you}\cite{heo2019fooling} itself to craft the incorrect explanations. 
%









==> oldrealted.tex <==
Efforts to improve the transparency of ML models can present significant privacy challenges. It has been shown in the literature that an adversary can misuse explanations to launch MIA \cite{shokri2021privacy}, model reconstruction \cite{milli2019model} \cite{aivodji2020model}, model inversion \cite{zhao2021exploiting}, and sensitive attribute inference \cite{duddu2022inferring} attacks. Our focus in this paper is on MIAs. In the literature, based on the construction of the attack model, MIA can be categorized into three major types, i.e., binary classifier-based attack approaches, metric-based attack approaches, and differential comparisons-based attacks.

\begin{enumerate}
    \item \textbf{Binary classifier-based attack approaches. }Essentially, a binary classifier-based MIA involves training a binary classifier, which can distinguish a target model’s training members' behavior from that of non-members. An effective technique called shadow training proposed by Shokri et al. \cite{shokri2017membership} is the first and perhaps the most widely used approach for training a binary classifier-based MIA. The main idea is that an attacker can create multiple shadow models to mimic the behavior of the target model because the attacker is assumed to know the target model's structure and learning algorithm. It can be of two types: white box \cite{shokri2017membership, salem2018ml, yeom2018privacy, hui2021practical} and black box \cite{nasr2019comprehensive, melis2019exploiting, leino2020stolen}. Meanwhile, in black-box, an attacker can only have black-box access to a target model.
    
    \item \textbf{Metric-based attack approaches. }Unlike binary classifier-based MIAs relying on training a binary classifier to recognize the complex relationship between members and nonmembers, metric-based MIAs \cite{long2017towards, salem2018ml, yeom2018privacy} are more simple and less computational. Metric-based MIAs make membership inference decisions for data records by first calculating metrics on their prediction vectors. The calculated metrics are then compared with a preset threshold to decide the membership status of the data record. The metric-based attack approaches again can be divided into the following categories:

    \noindent
    \textbf{Prediction Correctness-based MIA \cite{yeom2018privacy}. }An attacker infers an input record x as a member if it is correctly predicted by the target model, otherwise the attacker infers it as a non-member. The intuition is that the target model is trained to predict correctly on its training data, which may not generalize well on the test data.
    
    \textbf{Prediction Loss-based MIA \cite{yeom2018privacy}. }An attacker infers an input record as a member if its prediction loss is smaller than the average loss of all training members, otherwise the attacker infers it as a non-member. The intuition is that the target model is trained on its training members by minimizing their prediction loss.

    \textbf{Prediction Confidence-based MIA \cite{salem2018ml}. }An attacker infers an input record as a member if its maximum prediction confidence is larger than a preset threshold, otherwise the attacker infers it as a non-member. The intuition is that the target model is trained by minimizing prediction loss over its training data, which means the maximum confidence score of a training member’s prediction vector should be close to 1.

    \textbf{Prediction Entropy-based MIA \cite{salem2018ml}. }An attacker infers an input record as a member if its prediction entropy is smaller than a preset threshold, otherwise the attacker infers it as a nonmember. The intuition is that the prediction entropy distributions between training and test data are very different.

    \textbf{Modified Prediction Entropy-based MIA \cite{song2021systematic}. }The authors in Reference \cite{song2021systematic} argue that the existing prediction entropy-based MIA does not consider any information about the ground truth label, which might misclassify members and non-members.
      
    \item \textbf{Differential comparisons-based attacks. }Authors in \cite{hui2021practical}, an ML model is trained in a differentially private manner, the learned model does not learn or remember any specific user’s details if the privacy budget is sufficiently small. By definition, differenitially private models naturally limit the success probability of MIAs based solely on the model. We propose an MI attack, called BLINDMI, which probes the target model and extracts membership semantics via a novel approach, called differential comparison. The high-level idea is that BLINDMI first generates a dataset with nonmembers via transforming existing samples into new samples, and then differentially moves samples from a target dataset to the generated, non-member set in an iterative manner. If the differential move of a sample increases the set distance, BLINDMI considers the sample as non-member and vice versa.
    
\end{enumerate}

Game-theoretic approaches, such as zero-sum games \cite{dekel2010learning} \cite{globerson2006nightmare}, non-zero sum games \cite{dritsoula2017game}, sequential Bayesian game \cite{zhou2014adversarial} \cite{grosshans2013bayesian}, sequential Stackelberg games \cite{bruckner2011stackelberg} \cite{alfeld2017explicit} and simultaneous game \cite{dalvi2004adversarial}, have been used in the research literature to model interactions with ML models, specifically to model adversarial classification. Contrary to these efforts, where an adversary's objective is to target the classification task of the ML model, our research effort focuses on the descriptive task of the ML model, i.e., explaining the model predictions.
We used a continuous-time stochastic Signaling game \cite{neyman2017continuous} \cite{brazdil2009continuous} \cite{averboukh2016approximate} \cite{sobel2020signaling} to model such interactions. To the best of our knowledge, there has been no work that utilizes game theory to study the privacy leakages that can occur due to model explanations. Generally, continuous-time stochastic Signaling games are used in economic theory to study: stock prices \cite{dixit2012investment}, dynamic limit pricing \cite{gryglewicz2009signaling} \cite{gryglewicz2019strategic}, and market trading \cite{daley2012waiting}. We use GBM \cite{reddy2016simulating} \cite{hu1998optimal} \cite{dixit2012investment} to model the explanations variance to analyze how an adversary can utilize historical variance information to reach the target variance threshold. Thus, it is  the first work that integrates concepts from economics theory into the domain of ML and explanation methods to study MIAs. \vspace{-0.2cm}


Efforts to improve the transparency of ML models can present significant privacy challenges. It has been shown in the literature that an adversary can misuse explanations to launch MIA \cite{shokri2021privacy}, model reconstruction \cite{milli2019model} \cite{aivodji2020model}, model inversion \cite{zhao2021exploiting}, and sensitive attribute inference \cite{duddu2022inferring} attacks. Our focus in this paper is on MIAs. In this attack, as it has been shown in \cite{shokri2021privacy}, high explanation variance values at any datapoint $\overrightarrow{x}$ indicates that $\overrightarrow{x}$ was not used for training the model or the model is uncertain about the prediction of $\overrightarrow{x}$ paving the way towards a potential attack by an adversary. However, this work \cite{shokri2021privacy} only analyzed the single ``what if" interaction scenario, i.e., if an adversary knows the optimal variance threshold and has access to half of the training data, what is the impact of different settings on MIA? In contrast, in our work, we improved upon this analysis by modeling repeated interactions between the \texttt{system} and the malicious \texttt{end-user} and then analyzed the impact of different settings on MIA using the obtained optimal strategies and the optimal variance thresholds.



binary classifier-based attack approaches \cite{shokri2017membership}. It can be of two types: white box \cite{shokri2017membership, salem2018ml, yeom2018privacy, hui2021practical} and black box \cite{nasr2019comprehensive, melis2019exploiting, leino2020stolen}. In white-box setting, an attacker can get all the information and use it to attack a target ML model. The information includes the distribution of training data, how the target model is trained, and the architecture and the learned parameters of the target model. While, in black-box, an attacker can only have black-box access to a target model. The attacker is given information limited to training data distribution and black-box queries on the target model. \cite{leino2020stolen} Leveraging new insights about how overfitting occurs in deep neural networks, we show how a model’s idiosyncratic use of features can provide evidence for membership to white-box attackers—even when the model’s black-box behavior appears to generalize
well—and demonstrate that this attack outperforms prior black-box methods. 

    




Differential comparisons-based attack 



